On The Gap Between Software Maintenance Theory and Practitioners' Approaches

The way practitioners perform maintenance tasks in practice is little known by researchers. In turn, practitioners are not always up to date with the proposals provided by the research community. This work investigates the gap between software maintenance techniques proposed by the research community and the software maintenance practice. We carried out a survey with 112 practitioners from 92 companies and 12 countries. We concentrate on analyzing if and how practitioners understand and apply the following subjects: bad smells, refactoring, software metrics, and change impact analysis. This study shows that there is a large gap between research approaches and industry practice in those subjects, especially in change impact analysis and software metrics.

==> tables/aplicacao_vs_background.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!h]
\centering
\caption{p-values of Fisher's test for the association between practical application and participants' background}
\label{tab:rq3_2}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrr}
\hline
                                                                       & \multicolumn{3}{c}{\textbf{Participants' Background}}                                                                                                                                                                                                     \\ \cline{2-4} 
\textbf{Practical application}                                          & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Academic\\ Background\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Professional \\ Experience\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Company \\ Size\end{tabular}} \\ \hline
Software metrics                                                       & 0.99                                                                              & 0.99                                                                                   & 0.95                                                                        \\
Refactoring                                                            & 0.33                                                                              & \cellcolor[HTML]{67FD9A}\textbf{0.04}                                                  & 0.62                                                                        \\
Bad Smell                                                              & 0.90                                                                              & 0.16                                                                                   & 0.49                                                                        \\
\begin{tabular}[c]{@{}l@{}}Change Propagation\\  Analysis\end{tabular} & 0.42                                                                              & 0.25                                                                                   & 0.32                                                                        \\ \hline
\end{tabular}%
}
\end{table}

==> tables/familiaridade_vs_background.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!h]
\centering
\caption{p-values of Fisher's test for the association between familiarity and participants' background}
\label{tab:rq3_1}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lrrr}
                                                                      & \multicolumn{3}{c}{\textbf{Participants' Background}}                                                                                                                                                                                                     \\ \cline{2-4} 
\textbf{Familiarity}                                                  & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Academic \\ Background\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Professional \\ Experience\end{tabular}} & \multicolumn{1}{l}{\begin{tabular}[c]{@{}l@{}}Company \\ Size\end{tabular}} \\ \hline
Software  Metrics                                                     & 0.84                                                                               & 0.65                                                                                   & 0.51                                                                        \\
Refactoring                                                           & 0.43                                                                               & 0.48                                                                                   & 0.21                                                                        \\
Bad Smell                                                             & 0.18                                                                               & \cellcolor[HTML]{DAE8FC}\textbf{0.09}                                                  & \cellcolor[HTML]{DAE8FC}\textbf{0.06}                                       \\
\begin{tabular}[c]{@{}l@{}}Change Propagation\\ Analysis\end{tabular} & \cellcolor[HTML]{DAE8FC}\textbf{0.07}                                              & 0.71                                                                                   & 0.27                                                                        \\ \hline
\end{tabular}%
}
\end{table}



==> tables/opcoes_resposta_bk.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[h!]
\caption{ Reply options about practitioners’ background}
\label{tab:background}
\resizebox{\linewidth}{!}{%
\begin{tabular}{p{3cm}p{7cm}}

\multicolumn{1}{c}{Background}     & \multicolumn{1}{c}{Reply Options}                                                                                        \\ \midrule
Academic Background                & High school, Technician, Undergraduate degree, Specialization course, Master’s degree, or Doctorate degree       \\
Professional Experience            & up to 2 years, more than 2 up to 5 years, more than 5 up to 10 years, more than 10 up to 15 years, or more than 15 years \\
Company Size & up to 9, from 10 to 49, from 50 to 249, or 250 or more                                                                   \\ \midrule
\end{tabular}%
}
\end{table}

==> tables/tabelaRQ3.tex <==

\begin{table*}[h]
\centering
\caption{Fisher's test p-values}
\label{tab:p-values}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lrrrllrrr@{}}
\cmidrule(r){1-4} \cmidrule(l){6-9}
                            & \multicolumn{3}{c}{\textbf{Participants' Backgrond}}                                                                             &  &                               & \multicolumn{3}{c}{\textbf{Participants' Backgrond}}                                                                             \\ \cmidrule(lr){2-4} \cmidrule(l){7-9} 
\textbf{Familiarity}        & \multicolumn{1}{l}{Academic Background} & \multicolumn{1}{l}{Professional Experience (years)} & \multicolumn{1}{l}{Company size} &  & \textbf{Pratical application} & \multicolumn{1}{l}{Academic Background} & \multicolumn{1}{l}{Professional Experience (years)} & \multicolumn{1}{l}{Company size} \\ \cmidrule(r){1-1} \cmidrule(lr){6-6}
Software metrics            & 0.68                                    & 0.65                                                & 0.38                             &  & Software metrics              &                                         &                                                     &                                  \\
Refactoring                 & 0.48                                    & 0.72                                                & 0.51                             &  & Refactoring                   &                                         &                                                     &                                  \\
Bad Smell                   & 0.26                                    & 0.065                                               & 0.14                             &  & Bad Smell                     &                                         &                                                     &                                  \\
Change Propagation Analysis & \cellcolor[HTML]{CBCEFB}\textbf{0.07}   & 0.7                                                 & 0.27                             &  & Change Propagation Analysis   &                                         &                                                     &                                  \\ \cmidrule(r){1-4} \cmidrule(l){6-9} 
\end{tabular}%
}
\end{table*}
